In-Hand Manipulation of Unknown Objects with Tactile Sensing for Insertion

In this paper, we present a method to manipulate unknown objects in-hand using tactile sensing without relying on a known object model. In many cases, vision-only approaches may not be feasible; for example, due to occlusion in cluttered spaces. We address this limitation by introducing a method to reorient unknown objects using tactile sensing. It incrementally builds a probabilistic estimate of the object shape and pose during task-driven manipulation. Our approach uses Bayesian optimization to balance exploration of the global object shape with efficient task completion. To demonstrate the effectiveness of our method, we apply it to a simulated Tactile-Enabled Roller Grasper, a gripper that rolls objects in hand while collecting tactile data. We evaluate our method on an insertion task with randomly generated objects and find that it reliably reorients objects while significantly reducing the exploration time.

==> controller.tex <==
\subsection{Controller} \label{Controller}
We use the handcrafted controller from \cite{yuan2020design} to determine the roller pitch angle and roller velocity necessary to achieve the desired rotation of the object. The controller makes the assumption that the object is a sphere, but we find that by adding compliance to the opening of the roller grasper, we can reorient a broader set of object shapes beyond spheres. However, due to the geometry of the roller grasper, it is physically impossible to manipulate objects with a large aspect ratio in any direction, so we limit ourselves to objects with aspect ratios close to 1. 

==> znotes.tex <==
An example of paper that used "insertion task" with "peg insertion" only used to refer to a specific instance:
"Meta-Reinforcement Learning for Robotic Industrial Insertion Tasks"
https://ieeexplore.ieee.org/abstract/document/9340848


